Interactive Open-Ended Learning for 3D Object Recognition

The thesis contributes in several important ways to the research area of 3D object category learning and recognition. To cope with the mentioned limitations, we look at human cognition, in particular at the fact that human beings learn to recognize object categories ceaselessly over time. This ability to refine knowledge from the set of accumulated experiences facilitates the adaptation to new environments. Inspired by this capability, we seek to create a cognitive object perception and perceptual learning architecture that can learn 3D object categories in an open-ended fashion. In this context, ``open-ended'' implies that the set of categories to be learned is not known in advance, and the training instances are extracted from actual experiences of a robot, and thus become gradually available, rather than being available since the beginning of the learning process. In particular, this architecture provides perception capabilities that will allow robots to incrementally learn object categories from the set of accumulated experiences and reason about how to perform complex tasks. This framework integrates detection, tracking, teaching, learning, and recognition of objects. An extensive set of systematic experiments, in multiple experimental settings, was carried out to thoroughly evaluate the described learning approaches. Experimental results show that the proposed system is able to interact with human users, learn new object categories over time, as well as perform complex tasks. The contributions presented in this thesis have been fully implemented and evaluated on different standard object and scene datasets and empirically evaluated on different robotic platforms.

==> chapters/abstract_p2.tex <==
Open-ended learning for 3D object category recognition is the core problem in this thesis. Two learning approaches were explored for incrementally scaling-up to larger sets of categories. Finally, a novel experimental evaluation methodology, that takes into account the open-ended nature of object category learning in multi-context scenarios, is proposed and applied. An extensive set of systematic experiments, in multiple experimental settings, was carried out to thoroughly evaluate the described learning approaches. The results indicate that all approaches were able to incrementally acquire new categories. 

The contributions presented in this thesis have been fully implemented and evaluated on different standard object and scene datasets and empirically evaluated on different robotic platforms. Experimental results show that the proposed system is able to interact with human users, learn new object categories over time, as well as perform complex tasks.

==> chapters/abstract_pt.tex <==
Current object category learning and recognition approaches are often designed for static environments in which it is viable to separate the training (off-line) and testing (on-line) phases. In these cases, the learned object category models are static, in the sense that the representation of the known categories does not change after the training stage. Moreover, to migrate a robot to a new environment one must often completely redesign and remodel the knowledge-base that it is running with. 

The thesis contributes in several important ways to the research area of 3D object category learning and recognition. To cope with the mentioned limitations, we look at human cognition, in particular at the fact that human beings learn to recognize object categories ceaselessly over time. This ability to refine knowledge from the set of accumulated experiences facilitates the adaptation to new environments. Inspired by this capability, we seek to create a cognitive object perception and perceptual learning architecture that can learn 3D object categories in an open-ended fashion. In this context, ``open-ended'' implies that the set of categories to be learned is not known in advance, and the training instances are extracted from actual experiences of a robot, and thus become gradually available, rather than being available since the beginning of the learning process. In particular, this architecture provides perception capabilities that will allow robots to incrementally learn object categories from the set of accumulated experiences and reason about how to perform complex tasks. This framework integrates detection, tracking, teaching, learning and recognition of objects. 

An important part of this work is concerned with the object representation. This is one of the most challenging problems in robotics because it must provide reliable information in real-time to enable the robot to physically interact with the objects in its environment. We have first tackled the problem of object representation, by proposing a new global object descriptor named Global Orthographic Object Descriptor (GOOD) designed to be robust, descriptive and efficient to compute and use. GOOD distinguishes itself from alternative 3D global object representations in that it is very fast to compute, robust against variations in pose and sampling density, and copes well with noisy sensor data. We also propose an extension of Latent Dirichlet Allocation to learn structural semantic features (i.e. topics) from local feature co-occurrences for each object category independently. Although the model we developed has been intended to be used for object category learning and recognition, it is a novel probabilistic model that can be used in the fields of computer vision and machine learning.  

Open-ended learning for 3D object category recognition is the core problem in this thesis. Two learning approaches were explored for incrementally scaling-up to larger sets of categories. Finally, a novel experimental evaluation methodology, that takes into account the open-ended nature of object category learning in multi-context scenarios, is proposed and applied. An extensive set of systematic experiments, in multiple experimental settings, was carried out to thoroughly evaluate the described learning approaches. 
Experimental results show that the proposed system is able to interact with human users, learn new object categories over time, as well as perform complex tasks. The contributions presented in this thesis have been fully implemented and evaluated on different standard object and scene datasets and empirically evaluated on different robotic platforms. 




==> chapters/bibliography.tex <==
\chapter{}

\bibliographystyle{apalike}
\bibliography{bib/all_refs,new}


==> packages.tex <==
%load any additional packages
%\usepackage{times}
\usepackage{amssymb}
\usepackage[hidelinks]{hyperref}
\usepackage{color}
\usepackage{chngcntr}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{listings}
\usepackage{courier}
\usepackage{soul}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{subfigure}% Support for small, `sub' figures and tables
\usepackage{multirow}
\usepackage{graphicx}
\usepackage[flushleft]{threeparttable}
\usepackage{booktabs}
\usepackage{flushend}
% \usepackage{etoolbox}
\usepackage{fixltx2e} % for superscript and subscript textcolor
\usepackage{bm}
\usepackage{amsfonts}
\usepackage[T1]{fontenc}
% \usepackage{lmodern}
\usepackage{enumitem}
\usepackage{tabularx}
\usepackage{array}
\usepackage{placeins}
\usepackage{rotating}

\usepackage{float}
\floatstyle{plain}
\newfloat{lstfloat}{tbp}{lop}
\floatname{lstfloat}{Listing}
\def\lstfloatautorefname{Listing} % needed for hyperref/auroref


%% adding the end marks
\usepackage{amsthm}
\usepackage{thmtools}
\declaretheorem[style=definition,qed={\small$\blacksquare$},numberwithin=chapter]{definition}
\declaretheorem[style=definition,qed={\small$\square$},numberwithin=chapter]{example}
% \declaretheorem[style=definition,qed=$\blacktriangle$,numberwithin=chapter]{example}
\declaretheorem[style=definition,qed={\small$\blacksquare$},numberwithin=chapter]{function}
% \declaretheorem[style=definition,qed={\small$\blacksquare$},numberwithin=chapter]{method}

\declaretheorem[style=plain,sibling=definition]{theorem}
\declaretheorem[style=plain,sibling=definition]{lemma}
%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Roman: this defines \cupdot
\makeatletter
\def\moverlay{\mathpalette\mov@rlay}
\def\mov@rlay#1#2{\leavevmode\vtop{%
   \baselineskip\z@skip \lineskiplimit-\maxdimen
   \ialign{\hfil$\m@th#1##$\hfil\cr#2\crcr}}}
\newcommand{\charfusion}[3][\mathord]{
    #1{\ifx#1\mathop\vphantom{#2}\fi
        \mathpalette\mov@rlay{#2\cr#3}
      }
    \ifx#1\mathop\expandafter\displaylimits\fi}
\makeatother

\newcommand{\cupdot}{\charfusion[\mathbin]{\cup}{\cdot}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros}


%% to ignore greek letters in mathcal >>
\DeclareMathSymbol{\Gamma}{\mathord}{operators}{"00}
\DeclareMathSymbol{\Delta}{\mathord}{operators}{"01}
\DeclareMathSymbol{\Theta}{\mathord}{operators}{"02}
\DeclareMathSymbol{\Lambda}{\mathord}{operators}{"03}
\DeclareMathSymbol{\Xi}{\mathord}{operators}{"04}
\DeclareMathSymbol{\Pi}{\mathord}{operators}{"05}
\DeclareMathSymbol{\Sigma}{\mathord}{operators}{"06}
\DeclareMathSymbol{\Upsilon}{\mathord}{operators}{"07}
\DeclareMathSymbol{\Phi}{\mathord}{operators}{"08}
\DeclareMathSymbol{\Psi}{\mathord}{operators}{"09}
\DeclareMathSymbol{\Omega}{\mathord}{operators}{"0A}

%% declare mathpzc
\DeclareFontFamily{OT1}{pzc}{}
\DeclareFontShape{OT1}{pzc}{m}{it}{<-> s * [1.20] pzcmi7t}{}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

%% declare mathscr
\DeclareFontFamily{U}{mathc}{}
\DeclareFontShape{U}{mathc}{m}{it}{<->s*[1.03] mathc10}{}
\DeclareMathAlphabet{\mathscr}{U}{mathc}{m}{it}

%% declare mathscr
\DeclareMathAlphabet{\mathcalligra}{T1}{calligra}{m}{n}

%% declare italic sans serif
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\newcommand{\msi}[1]{\mathsfit{#1}}

\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mz}[1]{\mathpzc{#1}}
\newcommand{\ms}[1]{\mathsf{#1}}
\newcommand{\mcg}[1]{\mathcalligra{#1}}
\newcommand{\mcr}[1]{\mathscr{#1}}
%% to ignore greek letters in mathcal <<


%\newtheorem{definition}{Definition}

%% define ebpd term
\newcommand{\ebpd}{$\ms{EBPD}$}
\newcommand{\ebpds}{$\ms{EBPDs}$}

%% define colors
\definecolor{red}{rgb}{1.00,0.00,0.00}
\definecolor{blue}{rgb}{0.00,0.00,1.00}
\definecolor{green}{rgb}{0.4,1.00,0.0}
\definecolor{yellow}{rgb}{0.5,0.5,0.0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{ipython_frame}{RGB}{207, 207, 207}
\definecolor{halfgray}{gray}{0.3}
\newcommand{\cred}[1] {\textcolor{red}{#1}}
\newcommand{\cblue}[1] {\textcolor{blue}{#1}}
\newcommand{\cgreen}[1] {\textcolor{green}{#1}}
\newcommand{\cyellow}[1] {\textcolor{yellow}{#1}}

\algrenewcommand\alglinenumber[1]{\tiny\color{black} #1~}

\hyphenation{opera-tor ins-truc-tions frame-work key-pro-positions 
key-propo-sitions key-pro-per-ties}

\pdfinfo{
/Title (Gathering and Conceptualizing Plan-Based Robot Activity 
Experiences for Long-Term Competence Enhancement)
/Author (Vahid Mokhtari, Luis Seabra Lopes and Armando J. Pinho)
% /Subject (Robot task learning from experience)
% /Keywords (Learning from demonstration; Robot task learning; 
% Learning and planning; Conceptualization; Loop detection; Adaptability)
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\lstdefinestyle{customlst}{
    mathescape,
    %linewidth=.8\textwidth,
    %xleftmargin=.1\textwidth,
    %xleftmargin=3.4pt,
    %xrightmargin=3.4pt,    
    %framexleftmargin=-10mm,
    %framexrightmargin=-10mm,
    %frame=bt,
    %aboveskip=4pt, 
    %belowskip=6pt, 
    %rulecolor=\color{ipython_frame},
    %frame=tb,
    %frameround={t}{t}{t}{t},
    numbers=left,
    numbersep=-5.5pt, 
    numberstyle=\tiny\color{halfgray},
    captionpos=b,
    abovecaptionskip=10pt,
    %belowcaptionskip=-5pt,
    stepnumber=1,
    basicstyle=\ttfamily\fontsize{9}{8}\selectfont, 
    keywordstyle=\bfseries,
    morekeywords={properties}
    }
%\lstset{style=customlst}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% Chapter name in the header
\usepackage{fancyhdr}
\pagestyle{fancy}

\renewcommand{\chaptermark}[1]{\markboth{#1}{}}

\fancyhf{} % clear the headers
\fancyhead[R]{%
   % We want italics
   \itshape
   % The chapter number only if it's greater than 0
   \ifnum\value{chapter}>0 \chaptername\ \thechapter. \fi
   % The chapter title
   \leftmark}
\fancyfoot[C]{\thepage}

\fancypagestyle{plain}{
  \renewcommand{\headrulewidth}{0pt}
  \fancyhf{}
  \fancyfoot[C]{\thepage}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

